The Milky Way's Supermassive Black Hole: How good a case is it? A Challenge for Astrophysics & Philosophy of Science

The compact and, with 4.3+-0.3 million solar masses, very massive object located at the center of the Milky Way is currently the very best candidate for a supermassive black hole (SMBH) in our immediate vicinity. The strongest evidence for this is provided by measurements of stellar orbits, variable X-ray emission, and strongly variable polarized near-infrared emission from the location of the radio source Sagittarius~A* (SgrA*) in the middle of the central stellar cluster. If SgrA* is indeed a SMBH it will, in projection onto the sky, have the largest event horizon and will certainly be the first and most important target of the Event Horizon Telescope (EHT) Very Long Baseline Interferometry (VLBI) observations currently being prepared. These observations in combination with the infrared interferometry experiment GRAVITY at the Very Large Telescope Interferometer (VLTI) and other experiments across the electromagnetic spectrum might yield proof for the presence of a black hole at the center of the Milky Way. It is, however, unclear when the ever mounting evidence for SgrA* being associated with a SMBH will suffice as a convincing proof. Additional compelling evidence may come from future gravitational wave observatories. This manuscript reviews the observational facts, theoretical grounds and conceptual aspects for the case of SgrA* being a black hole. We treat theory and observations in the framework of the philosophical discussions about "(Anti)Realism and Underdetermination", as this line of arguments allows us to describe the situation in observational astrophysics with respect to supermassive black holes. Questions concerning the existence of supermassive black holes and in particular SgrA* are discussed using causation as an indispensable element. We show that the results of our investigation are convincingly mapped out by this combination of concepts.

==> reply-refreport.tex <==


Dear Carlo;
Please find attached our response to the referee's and your comments.
We worked on all points and highlighted the changes in bold face 
letters.
We are grateful for the comments and think that the paper has 
now gained in clarity and comprehension.

We hope that the paper now qualifies for being accepted.

All the best

Andreas Eckart

-----------------------------------------------------------------------------
> Referee A (Astrophysics):
>
> 
> SMBHs are philosophically interesting as they are only observable by indirect
>  means and suffer of “under-determination”. This is true, but it will remain 
> true only until LISA will fly. The SMBH hypothesis will be tested with 
> .......

LISA and gravitational wave are now mentioned at several positions in the paper.

We tried to improve on style and typo-situation.


>Specific comments:
> 
>Section 2 and 4.13:
>The role of the new astrophysics with GWs is mentioned in a 
>rather confused manner  in various places of the review.SMBH 
>spectroscopy during the ring-down of a merger and EMRIs will 
>become the main tool for testing rivaling theories on the 
>SMBH hypothesis, in completely different settings and the 
>closest to SgrA* is the case of EMRIs.
>Pulsars and stars probe the space time around SgrA*, which is a stationary.
>IMRIs are interesting as well but the signal is not known and 
>I would refrain from referring to a case which is still very 
>difficult to describe in GR.

IMRIs now not mentioned in that context

>The authors ignore three important reviews on this matter which 
>touch issues that are not side issues for this review:
>1.     “Testing GR with present and future astrophysical 
>observations” by Bert et al.  Classical and Quantum Gravity, 
>Volume 32, Issue 24, article id. 243001 (2015). There are 
>several alternative theories of gravity that predict the 
>existence of BHs.  How good would be the case of SgrA*, to 
>test these in the stationary sector?
>2.     “Testing GR with low-frequency space-based GW 
>detectors” by Gair et al., Living Review 2013.
>3.     “GW tests of GR and ground-based detectors and pulsar 
>timing array”, by Yunes et al. 2013, Living Review.
>These reviews should be cited. 

These three references are now mentioned.

> 
>Page 5:
>I am aware of the huge literature in this field, but I would 
>at least cite here the key review by Kormendy & Ho, 
>Annual Review of Astronomy and Astrophysics, vol. 51, 
>issue 1, pp. 511-653, after Ferrarese citation.

now mentioned
 
>Strong gravitational wave signals occur during the 
>final phase of the merging
>process (see the detection of gravitational waves from 
>binary stellar sources by the
>LIGO and Virgo collaborations Abbott et al, 2016) and might be 
>detected with Pulsar
>Timing Arrays (e.g. Wyithe and Loeb, 2003; Roedig and Sesana, 2012; 
>Pollney and Reisswig, 2011) in the future. Black holes play an 
>increasingly important role
>in many areas of astrophysics. Therefore, more pressing seems to 
>be the question:
>How good a case is it?

all these references were already in the paper at a location 
at which LIGO is mentioned first.

> 
>The discovery of GW150914 by the LIGO detectors is so important 
>for the matter discussed here that a citation within brackets 
>seems rather inappropriate. True that GW150914 is a stellar 
>origin BH, but incoming observations of BH coalescence are 
>destined to shed light on the nature of this type of objects 
>and test GR to high levels.
>Pulsar Timing Array will detect the foreground of GWs resulting 
>from the incoherent superposition of  inspiralling SMBH binaries 
>decades, years or months prior to merging, i.e. far from 
>coalescence, and thus can not provide any information to reduce 
>the level of “under-determination”.   The citation on PTA here 
>is inappropriate. But, LISA will detect SMBHs at coalescence 
>(please cite the white paper: The Gravitational Universe arXiv:1305.572). 
>These are BHs of the same mass of the BH at the GC. 
>Indeed, Sgr A* is the SMBH prototype for LISA.  LISA will have 
>the highest sensitivity just in the mass range between 10^5 – a few 10^6 
>solar masses.  This should be stated clearly.

We clarified this in the text and stated it clearly


>I invite the authors to read the paper by Berti et al: 
>“Spectroscopy of Kerr black holes with Earth- and space-based 
>interferometers”2016, Physical Review Letters, Volume 117, 
>Issue 10, id.101102. GW astrophysics is in its infancy, but the 
>ability to carry on gravitational wave spectroscopy” can not be 
>ignored when talking of “under-determination”. 
>I would advise to elaborate more on this point, otherwise the review 
>loses its relevance (as discussed above). The cooperative efforts 
>coming from say “classical” astronomy, and the “new GW astronomy” 
>will at the end be able to resolve the puzzle on the 
>nature of “the astrophysical black holes”.  

This is now mentioned in the framework of under-determination in section 3.1.
 
>In Section 4.4 I think that the authors should quote the key 
>paper by Merritt, Alexander, Mikkola & Will: 
>Testing properties of the GCBH using stellar orbits, Phys. Rev D, 81, 2010.

now done right before equation 13

>Section 4.13:
>This section needs a bit of re-wording, EMRIs are quoted at the 
>beginning and redefined in the third sentence. There are also 
>confusing concepts.
>Customarily, “ringing” is the word used to describe the ring-down 
>of the new SMBH formed in the aftermath of a SMBH binary merger. 
>It seems a bit inappropriate to refer to the inspiral and plunge 
>of an EMRI as a ringing of space time, being spacetime only weakly 
>perturbed.  Appendix B does not describe the fact that form 
>EMRIs the effective metric perturbation is not just h, but h 
>times the square root of the number of cycles the EMRI spends in band. 
>I do not  know if the luminosity of 10^40 erg/s is computed correctly. 
>Please check.

We now explain to clarify:

In a strict sense the word 'ringing' is used to describe the ring-down
of the new SMBH formed in the aftermath of a SMBH binary merger.
For simplicity we use it here for the gravitational wave signal we receive
from inspiralling masses.

We checked the calculation
 
>Concerning fermion balls in section 5.1:   fermion balls
> counterbalance gravity with the degeneracy pressure of the fermions. 
>I find a bit of a contradiction citing the Newtonian Lane-Endem 
>equation and at the same time the Oppenheimer Volkoff limit 
>which is the limit for relativistic stars in GR. Is the maximum 
>mass of fermion balls determined by the change in level of 
>degeneracy (from non- to ultra-relativistic) or simply due to GR? 
>I find this confusing.

Non-relativistic and relativistic descriptions are now clearly separated.
Such the non-relativistic is clearly attributed to the Lane-Endem
equation and relativistic is clearly attributed to the 
Oppenheimer Volkoff limit.
 
>I further do not understand why the limit imposed on the neutrino 
>mass by S2 implies Newtonian precession. Since no precession 
>is observed at the level of accuracy of current EM observations, 
>the radius of the neutrino ball should be inside the S2 orbit, 
>and this poses a limit on the neutrino mass (presumably 
>radius of the star). It seems instead that S2 is orbiting 
>inside the fermion ball.   I think that the authors need to better 
>rephrase this sentence and clear up section 5.1. 
>If fermion balls are extended objects, this should be stated clearly.

This has now been rephrased and better explained.
 
>A general comment:
>The BH hypothesis for explaining the presence of massive dark 
>objects at the centers of galactic nuclei is the most elegant 
>and simple. Fermion balls and boson balls can exist stably 
>only below a given (yet unknown) “maximum” mass, and for the case 
>of boson stars, bosons need to be dissipative and repulsive  
>in order to form the dark star.  
>However, in stellar astrophysics, two limiting masses exists: 
>the Chandrasekhar mass and the OV maximum mass for a neutron 
>stars of about 3 Msun.   In the context of stellar astrophysics, 
>we do see white dwarfs, neutron stars and stellar black holes, 
>i.e. transitions between the three different states. 
>Thus I would not in principle exclude the possibility to have 
>equilibria with a surface (as fermion or/and boson balls)  
>that become unstable forming  a SMBH when driven above a mass limit.

correct - but having a neutrino mass for each different SMBH is not
very satisfactory.

>Table 3 is an interesting summary table:
>“This table lists the necessary conditions that can be 
>combined to result in sufficient conditions required to 
>identify SgrA* as a SMBH, in the realm of EM observations.”

not exclusively EM: 'ringing' is included 

>More than necessary conditions in my view these are just necessary 
>tools, since in order to identify SgrA* as a SMBH we need not 
>only to have consistency in the mass and size measurements 
>from different EM methods but to probe with extremely high accuracy 
>that the structure of the spacetime around SgrA* is that predicted by Kerr.

yes - this is why more elaborate combinations of these constraints
only give useful results.

> A9) is a clear example: pulsars and stars are tools: I would not 
>consider this as a logical entity. I would not attribute 
>to A9) the state of being  “false” or “true”. It just depend 
>on the unknown stellar distribution. I may have missed the point 
>but I think that this is a bit misleading, though the text in 
>pages 39-44 tries to explain this better.
 
Agreed: A9 now renamed to :  
Do stars and pulsars close to SgrA* give indications for a SMBH? 

>Along these lines I do not understand why  conditions A_n are 
>phrased as questions:
>“Do we detect pulsars?” – I would just say “Detection of pulsars 
>within a given distance of 100M-1000M”. 

It says '... close to' and the size scales are discussed in the text.
As these items are going to be logically linked together one must
be able to attribute to them a yes/no true/false 0/1 value. 
For questions this comes quite naturally.

>A1) Is the object at the nominal position of SgrA*?
>Frankly, this is not a condition but in my this is the key 
>assumption necessary to initiate the whole process of 
>identification of SrgA* as a SMBH,

No, this is a condition. It is highly nontrivial. 
Activity may arise from close to the SMBH but may not necessarily
fully related to it (i.e. in the jet or out/inflow).
Also: Combining results or methods from/at different wavelengths the 
position must be determined in a common positional reference frame.
The precision is wavelength dependant due to many technical and
physical aspects.
One may 'see' a jet component offset from the dynamical mass center
associated with the SMBH. All of this must be verified in a 
self-consistent way.

>A4) Does the distance to SgrA* place it at the center of the Milky Way?
>I do not understand this condition: as far as I know there 
>are limits on the motion of SgrA* of a few km/sec.  
>But this is not a necessary condition to identify SgrA* as a SMBH, 
>in my view. A SMBH can be displaced (if e.g. is resulting 
>from a merger) and its center of mass may not strictly coincide 
>with the photometric center of the hosting bulge which is also 
>very difficult to define observationally.  There are attempts 
>to measure the displacement in the position of the SMBH in 
>M87 to infer whether it is a result of a merger, 
>being  M87 a very massive elliptical.

yes - sure - but all size scales, luminosities and 
physical velocities  derived from proper motions depend on the distance.
Hence, verifying the distance is essential if one wants to make use
of the observed properties, i.e. exceptionally high velocities or 
flare luminosities.
 
>A10) Is the spectrum of surrounding  SgrA* what is expected 
>from a SMBH? Do we really know the spectrum of the 
>surroundings of a SMBH?  Is it really “universal
>“ to make this statement so important?
>Why asking whether SgrA*  is a Kerr SMBH makes sense, since  
>this is a  key prediction of a fundamental theory of gravity as GR, 
>the surroundings of a SMBH likely depends on more complex processes 
>(presence of giant molecular  gas clouds, star formation,…), and the 
>spectrum may not be universal. I would not use this as a condition 
>to identify SgrA* as a SMBH.

correct - this condition cannot be used by itself but only in 
conjunction with additionally constraints. In the first 'manipulative
success' statement it is also clearly said that it must support the statement.
Universal: Depending on the accretion state certain expectations are
linked to the EM output of the surroundings of SMBHs.
As discussed in section '4.8 Does Sgr A* have a jet or an outflow?'
SgrA* is at the low luminosity end of low-luminosity AGN.
Hence, we would like to leave it in the list of conditions.
Also the spectrum of the surroundings is thought to be a function of the 
accretion state.
We now say at the beginning of section 4.6:

As in the case of stellar accreting black holes
the spectral properties of this region for accretion SMBHs
are intimately linked to the accretion state and the black hole location in
a fundamental plane expressing that state
\citep[e.g.][]{Markoff2011, Markoff2005, VasudevanFabian2007}.

 
>I like very much the idea of listing all different techniques that 
>can provide consistency in the measurement of the mass and size of 
>SgrA*, as  discussed in Section 6, and I think that B_8 (page 44) 
>(Psaltis & Kramer 2016) provides the best way to approach the problem.

Yes, that is also a result of the summary - however, it is also
not very likely to put it in place as we need to find suitable
stars and pulsars first.

>B_5 is very unlikely: the probability of getting the signal of an 
>EMRI (or possibly of an IMBH) is extremely low.  It is the confrontation 
>with future observations of other galactic nuclei which makes sense to quote.

correct - this is also what we state. However, it is difficult to
say (with a statistics of 1) if it is more likely to find a exceptional
accretion event, a sudden jet, a bright pulsar close to SgrA*,
or an EMRI signal.
We now say:
In this context it is the comparison to the
observational results for other galactic nuclei which may help to 
understand the situation for SgrA*.

> 
>****************************************************************************************
>
Referee B (Philosophy):

>As a philosopher of science especially physics, I can only really 
>assess Section 3, and the concluding Section 7. 
>
>The main strength of this paper is the detailed presentation 
>of the types of evidence, and their various combinations, that confirm, 
>or at least can claim to confirm!, the existence of an SMBH in SgrA*. 
>Thus Section 7 gives seven sufficient conditions B_1 to B_7 for 
>such confirmation: each a conjunction of some necessary conditions 
>(labeled as A_{\mu}). So far as I can tell, these seven conjunctions 
>and the discussion of them is sensible.
>
>As regards philosophy: 
>1) Section 3 is long and wayward in some respects. 
>It sometimes reads like a concatenation of personal notes 
>on/responses to some of the philosophical literature   
>2) I think Sec 3.2 and 3.3 could be, indeed should be, deleted entirely. 
>For ALL that the later discussion needs is the idea that we 
>confirm the existence of objects in space and time, i.e. empirical objects
>(as against the objects of pure mathematics, which are 
>causally inactive: which is the concern of Colyvan in his 1998 
>and in his book), by appropriate causal interaction  

In the Colyvan 1998 article (we refer to) the objects of 
pure mathematics are only a part of the examples that he treats. 
Other examples cover: prediction of the existance of planets,
weather predictions, prediction of the existance of elements.
It is in 'general' on the causality and not specificly 
only tuned to objects of pure mathematics.


>(successful manipulation/ successful causal investigation etc). 
>In particular, the details of the Eleatic Principle,  
>and of Fig 3, and even the causal closure of the empirical 
>world (for which, by the way: Ladyman 2009, p. 10 paragraph 5, 
>is a very odd reference!): these are NOT later used.

We removed the reference to Ladyman
and replaced it by a reference to Montero 2003.
We do not agree on the statement: '... these are NOT later used'.
There are several references to Fig.3 : sections 7, 8, footnote 25.
The causal principle enters in Fig.1 which is used and filled in
by specific items specific the the discussion in Fig. 13.

We cannot only remain with a section on "Realism/Underdetermination" and on
a formal logical approach as we still need to highlight the (as the referee 
correctly states) 'appropriate causal interaction':
We agree on suppressing sections 3.2 and 3.3 to some extent.
Hence, we have shortened the next two sections into the new section 
3.2 'The Involvement of Causality' and write:
The discussion on "Realism" and "Underdetermination" targets mainly the
consistency and repeatability of observations and in how far they provide
sufficient evidence to reliably support the validity of a theory.
As in all experiments discussed below (...) it is never the super massive black holes
themselves that are observed but only object that interact with it, e.g. gas, stars, light.
Hence, the evidence to reliably support the validity of a theory comes in through
causality described by the theory. ....

We have moved the remainder of the previous sections into the appendix
as we still think that the information collected  and evaluated in there
is useful for the reader and gives an additional background.
I case of Appendix B the text is not simply  a concatenation of 'personal notes'
but we have used italic script to structure the text for better 
comprehension. 
We ask the referee to permit the presentation of this information in the appendix.


>3) Section 3.1 on manipulability, Hacking etc: I recommend 
>considering the rich philosophical literature about instrumentation, 
>and experiment (e.g. Allan Franklin, at Colorado, several books; 
>Peter Galison, How Experiments End); and papers by Chris Smeenk 
>(Western Ontario). For the technical achievement of modern 
>galactic astronomy is truly amazing, as the data in the other 
>Sections bring out: none of that amazement, or philosophical 
>reflection about it, is in Section 3 as it stands now.

References to Franklin, Galison, and Smeenk
are now given at appropriate locations.

>4) Sec 3.4: the notation, and the language, could be made much 
>simpler and clearer. In particular:
>1. Write the necessary conditions as N_{\mu} not as A_{\mu}: 
>N is then mnemonic;
>2. Write the sufficient conditions as S_{\vu} not as B_{\nu}; 
>S is then mnemonic;

done

>Indeed the Greek indices are overdoing it: why not just i,j 
>(and sad to have \nu, which sounds like N, labeling the sufficient 
>conditions not the necessary ones)

We would like to stay with Greek letters.

>There are very many small errors of language or exposition:
>Examples about exposition:
>1. just above eq 5 p. 15: we have to assume the natural 
>numbers \nu and \mu are natural numbers/integers.
>2. This should just be: we will take \nu and \mu to be natural 
>numbers. (You never use negative, so why mention integers?)

fixed

>3. Table 3, p. 39, list of A1 to A14: These necessary conditions 
>should not be questions; they should be propositions/claims/sentences.	

since we connect them logically they need to have a defined value
true/false  yes/no 1/0 - putting the statements in the form of a question
this is provided naturally

>4. eq 5 p. 15; First double arrow: stating that B is equivalent 
>to the conjunction of the necessary conditions A: I think this 
>is never used! and it should be given up: it is general contentious, 
>if we consider necessary conditions you can really formulate/confirm. 
>Example: Look at Table 3, p. 39, list of A1 to A14: Suppose that 
>all of A1 to A14 are true, and ask: is that logically equivalent 
>to the existence of an SMBH? 
>Of course not: there is always room for skepticism. 
>Such skepticism may well be irrational, but it does imply that 
>the first double arrow  of eq 5 p. 15 must be wrong. 
>That is: it should only be a rightward arrow.

done

>Small errors of language: Examples:
>p. 10 paragraph 2 line 1: cannot say: bears; must say: faces.

done

>p. 11, Sec 3.2 start: in English, we do not say a theory is real : 
>we say it is true. So write: Theory taken literally as being true.

done

>p. 11 Sec 3.2parag 3 line 4: many literally reading philosophers: 
>that is not English.

changed

>p. 11 3 lines from bottom: explanatory out of theory: meaning unclear

changed

>p. 13 Fig 2 : symmetry, entities, causally and relying: all mis spelt.

sorry; corrected 

>p 39 paragraph 1 line 8: say: rely: not relay

done

>p. 40 7 lines from bottom: the verb ‘allow’ needs a person as 
>grammatical object. You cannot just say: will allow to independently etc.
>you must say: will allow us/one/physicists to independently etc

done

>p. 42 5 lines from bottom: need: a in Schwarzschild

done

>
>Substantial revisions is needed, as well as much more careful writing. 
>There are many spelling errors; but it is not just spelling errors!

*****************************************************************************************
 
>Referee C (comment from the editor):
>
>It would be good if the revision could clarify the three following 
>questions:

We tried to accomplish this:

>i) I do not understand why is a black hole to be considered an object 
>substantially different from an electron, or, for that matter, 
>from a chair.  

on electrons, galaxies, and chairs: see below

> In principle, a black hole could be produced in a 
>laboratory, we could play table tennis with it, it would leave 
>traces where it passes, like electrons and chairs. 
>In all three cases, we interact only very indirectly with the object: 
>we receive photons that have bounced out from the object, or similar. 

This is not true for supermassive black holes.
There is nothing emitted from supermassive black holes.
Gravitational wave ringing originates due to the imprint into spacetime 
in the immediate vicinity of merging SMBHs
(Hawking radiation is way to weak to be detected; as highlighted in the paper)

>I do not see what is the difference in principle. 
>Of course, in practice a black hole is much harder to produce 
>and manipulate than chairs, 

Not so for SMBHs

>but so is -say- a galaxy, about which 
>we do not ask the questions that are being asked about black holes here.  
>If we want to be realists about chairs (pace Hume), why not black holes?  
>If we want to be realists about galaxies (pace van Fraassen), 
>why not black holes? 

In the paper we now say:
Hence, black holes may be seen as the prototype of 
astrophysical entities that suffer from underdetermination.
There is however ample indirect evidence for their existence.



>ii) For any object in the universe we talk about, we have mental, 
>visual, and mathematical models that work more or less well.  
>To the extent they work well, we consider them good description 
>of the object. To the extent they do not work well, we look for others.  
>We also keep exploring alternatives even when our theories work well, 
>because this is good practice in science. 
>Is the paper saying that black holes are *different* in this respect? 
>If yes, I have not understood why.  If no, why doesn't the paper 
>say this clearly? In other words, is the analysis of the black hole 
>situation just a case study for an object like any others, 
>or does it indicates that black holes are somehow a category of 
>entities apart? If so, I am missing something. 
>If not, why not saying this clearly?

In the paper we say:
Underdetermination arises both from the rarity of the expected event and from
the fact that the observations alone can probably not clearly discriminate the black
hole case against possible alternatives. 

>iii) Classical general relativity predicts that black holes are 
>stable and that no signal from their interior can come out.  
>But we know virtually for sure that classical relativity is an 
>approximation that breaks down, and there is large theoretical 
>consensus that the infinite stability of black holes is only an 
>artefact of the classical approximation.  
>If so, the idea itself of event horizon is not to be taken 
>seriously as fundamental, and a gravitationally collapsed star is 
>just a phenomenon without any particularly distinguishing property.  
>The question then returns: what is so special about black holes, 
>to motivate a *philosophical* discussion about their reality, 
>above the usual *astrophysical* discussion of the correctness 
>of our models of phenomena? 

Placing this early in the text is difficult.
We now write towards the end of the introduction:

---
For the current paper it needs to be clarified
if supermassive black holes are
different entities compared to, .e.g., electrons, chairs, or galaxies,
such that a special consideration in the frame work of
philosophy of science is justified?
While all of them can be discriminated from each other in the
framework of an constructive empiricism
there are noteworthy differences:
Entities like chair or tables stand out with respect to the
imperfection of their definition
\citep[as outlined by, e.g. David Hume; see][]{Nelson2010},
Galaxies stand out with respect to their distance and complexity
\citep[these object have been considered by][]{vanFraassen1985},
and electrons are very simple entities that
can be "sprayed" \citep{Hacking1989},
i.e., they are readily available in the laboratory for causality test.
Black holes, and in particular supermassive black holes
stand out in the simplicity of their mathematical definition
that is best expressed in the "no-hair" theorem
(see section \ref{definition}).
They are not readily available in the laboratory and cannot
easily be "sprayed".
They are characterized by an event horizon, that, however, cannot
become part of an external observer's past in a finite time
but is an important discriminator against other
similarly compact and massive objects.

Claiming that black holes are only approximated by their description
in classical relativity and thereby
compromising on the seriousness with which we treat the event horizon,
makes the problem even worse. In this case it is even more difficult
to distinguish between the black hole solution and other descriptions of
compact objects of the same mass.
----

So in essence:
It is not really a discussion about their reality - but rather 
about the uniqueness with which we are (or will be) able to discriminate 
against other descriptions that are in agreement with the data.

> from your email:
> I have reread Sections 3.2 and 3.3 and indeed, .....

both sections are now merged into a common shorter one dealing with the 
inclusion of causality which is after all necessary.
The rest went into appendices - as the sections still contain 
important information.

> Colyvan's extension: if is true that Colyvan's concern is the existence of *mathematical* entities,....

In the Colyvan 1998 article (we refer to) the objects of pure mathematics are only a 
small part of the examples that he treats. It is in 'general' on the
causality and not specificly only tuned to objects of pure mathematics.
Other examples in Colyvan's article cover: 
prediction of the existance of planets,
weather predictions, prediction of the existance of elements.
It is in 'general' on the causality and not specificly 
only tuned to objects of pure mathematics.

*****************************************************************************************





==> text.tex <==


The Milky Way's Supermassive Black Hole: How good a case is it?
A Challenge for Astrophysics & Philosophy of Science


64 pages; 13 pages of references; 13 figures; 3 tables; 4 appendices;

Published by Springer in -Foundations of Physics-
The final publication is available at Springer via http://dx.doi.org/DOI: 10.1007/s10701-017-0079-2


Andreas Eckart,
Andreas Huettemann,
Claus Kiefer,
Silke Britzen,
Michal Zajacek,
Claus Laemmerzahle,
Manfred Stockler,
Monica Valencia-S.,
Vladimir Karas,
Macarena Garcia-Marin


The compact and, with about 4.3+-0.3 million solar masses,
very massive object located at the center of the Milky Way is
currently the very best candidate for a supermassive black hole (SMBH)
in our immediate vicinity.
If SgrA* is indeed a SMBH it will, in projection
onto the sky, have the largest
event horizon and will certainly be the first and most important
target for Very Long Baseline Interferometry (VLBI) observations currently 
being prepared by the Event Horizon Telescope (EHT).
These observations in combination with the infrared interferometry experiment GRAVITY
at the Very Large Telescope Interferometer (VLTI) and other experiments across the
electromagnetic spectrum might yield proof for the presence of a
black hole at the center of the Milky Way.
This manuscript reviews the observational facts, theoretical grounds
and conceptual aspects for the case of SgrA* being a black hole.
We treat theory and observations in the
framework of the philosophical discussions about 
``(Anti)Realism and Underdetermination",
as this line of arguments allows us to describe the situation in observational
astrophysics with respect to supermassive black holes.
Questions concerning the existence of supermassive black holes and in particular SgrA* are
discussed using causation as an indispensable element.
We show that the results of our investigation are convincingly mapped 
out by this combination of concepts.


keywords
Black Holes: mass, spin, charge 
Sources: Sagittarus~A* 
Galaxies: Active 
Philosophy of Science: (Anti)Realism, Underdetermination, Causality}

